The Kelvin-Helmholtz instability in the Orion nebula: The effect of radiation pressure

The recent observations of rippled structures on the surface of the Orion molecular cloud (Bern\'{e} et al. 2010), have been attributed to the Kelvin-Helmholtz (KH) instability. The wavelike structures which have mainly seen near star-forming regions taking place at the interface between the hot diffuse gas, which is ionized by massive stars, and the cold dense molecular clouds. The radiation pressure of massive stars and stellar clusters is one of the important issues that has been considered frequently in the dynamics of clouds. Here, we investigate the influence of radiation pressure, from well-known Trapezium cluster in the Orion nebula, on the evolution of KH instability. The stability of the interface between HII region and molecular clouds in the presence of the radiation pressure, has been studied using the linear perturbation analysis for the certain range of the wavelengths. The linear analysis show that consideration of the radiation pressure intensifies the growth rate of KH modes and consequently decreases the e-fold time-scale of the instability. On the other hand the domain of the instability is extended and includes the more wavelengths, consisting of smaller ones rather than the case when the effect of the radiation pressure is not considered. Our results shows that for $\lambda_{\rm KH}>0.15\rm pc$, the growth rate of KH instability dose not depend to the radiation pressure. Based on our results, the radiation pressure is a triggering mechanism in development of the KH instability and subsequently formation of turbulent sub-structures in the molecular clouds near massive stars. The role of magnetic fields in the presence of the radiation pressure is also investigated and it is resulted that the magnetic field suppresses the effects induced by the radiation pressure.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
